MLQE-PE: A Multilingual Quality Estimation and Post-Editing Dataset

We present MLQE-PE, a new dataset for Machine Translation (MT) Quality Estimation (QE) and Automatic Post-Editing (APE). The dataset contains eleven language pairs, with human labels for up to 10,000 translations per language pair in the following formats: sentence-level direct assessments and post-editing effort, and word-level good/bad labels. It also contains the post-edited sentences, as well as titles of the articles where the sentences were extracted from, and the neural MT models used to translate the text.

==> figures/figure_hist_all_langs.tex <==
\begin{figure*}[ht]
\centering
    \includegraphics[scale=0.5]{figures/histograms/all_langs.png}
\caption{Distribution of direct assessments and HTER scores for the test21 partition of the dataset}
\label{fig:histograms_high_resource_test21}
\end{figure*}


==> figures/histograms_big.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-sien-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-neen-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-roen-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-enzh-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-ende-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-ruen-da.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-enzh-hter.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-ende-hter.png}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/histograms/hist-eten-da.png}
\end{subfigure}
\caption{Distribution of direct assessment and HTER scores on the test partition of the dataset}
\label{fig:histograms}
\end{figure*}


==> figures/histograms_small.tex <==
\begin{figure*}[ht]
\centering
    \includegraphics[width=.7\textwidth]{figures/da_distribution_with_hter_test20_bins10.png}
\caption{Distribution of direct assessments and HTER scores for the test partition of the dataset}
\label{fig:histograms}
\end{figure*}

